RF-ULM: Ultrasound Localization Microscopy Learned from Radio-Frequency Wavefronts

In Ultrasound Localization Microscopy (ULM), achieving high-resolution images relies on the precise localization of contrast agent particles across a series of beamformed frames. However, our study uncovers an enormous potential: The process of delay-and-sum beamforming leads to an irreversible reduction of Radio-Frequency (RF) channel data, while its implications for localization remain largely unexplored. The rich contextual information embedded within RF wavefronts, including their hyperbolic shape and phase, offers great promise for guiding Deep Neural Networks (DNNs) in challenging localization scenarios. To fully exploit this data, we propose to directly localize scatterers in RF channel data. Our approach involves a custom super-resolution DNN using learned feature channel shuffling, non-maximum suppression, and a semi-global convolutional block for reliable and accurate wavefront localization. Additionally, we introduce a geometric point transformation that facilitates seamless mapping to the B-mode coordinate space. To understand the impact of beamforming on ULM, we validate the effectiveness of our method by conducting an extensive comparison with State-Of-The-Art (SOTA) techniques. We present the inaugural in vivo results from a wavefront-localizing DNN, highlighting its real-world practicality. Our findings show that RF-ULM bridges the domain shift between synthetic and real datasets, offering a considerable advantage in terms of precision and complexity. To enable the broader research community to benefit from our findings, our code and the associated SOTA methods are made available at https://github.com/hahnec/rf-ulm.

==> figures/fig_gap_analysis.tex <==
\begin{figure*}[h!]
\hfill
\begin{minipage}[b]{.235\linewidth}
    \includegraphics[width=\linewidth]{figures/fig_gap_analysis/close_gap.png}
    \subcaption{$g=1$}
\end{minipage}
\hfill
\begin{minipage}[b]{.235\linewidth}
    \includegraphics[width=\linewidth]{figures/fig_gap_analysis/mid_gap.png}
    \subcaption{$g=8$}
\end{minipage}
\hfill
\begin{minipage}[b]{.235\linewidth}
    \includegraphics[width=\linewidth]{figures/fig_gap_analysis/large_gap.png}
    \subcaption{$g=16$}
\end{minipage}
\hfill
\begin{minipage}[b]{.235\linewidth}
    \includegraphics[width=\linewidth]{figures/fig_gap_analysis/large_gap.png}
    \subcaption{$g=\{2,4,\dots,16\}$}
\end{minipage}
\caption{Impact of channel gaps on localization resolution at varying distances. The channel gap can be regarded as sub-aperture width or baseline in parallax terms. \label{fig:baseline_impact}}
\end{figure*}

==> figures/fig_invivo_rat18_single_col.tex <==
% https://tiborstanko.sk/closeups.html
% trim={<left> <lower> <right> <upper>}
\begin{figure*}%[H]
    \centering
    \begin{minipage}[b]{\linewidth}
    \resizebox{\textwidth}{!}{
        \begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
        \node[anchor=south,scale=1.5] (FigA) at (0,0) {
        \includegraphics[height=2cm,trim=4cm 11.67cm 3.33cm 1.67cm,clip]{figures/fig_invivo/rat18/unet_8x.png}
        };
        \spy [closeup,magnification=3] on ($(FigA)+(-0.465,+0.075)$) 
        in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.115,+0.020)$) 
        in node[largewindow,anchor=east]       at ($(FigA.west)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.435,-0.075)$) 
        in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
        \end{tikzpicture}
    }
    \subcaption{U-Net approach~\cite{van2020super} with NMS from upscaled B-mode frames\label{fig:rat18:subfig1}}
    \end{minipage}
    \begin{minipage}[b]{\linewidth}
    \resizebox{\textwidth}{!}{
        \begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
        \node[anchor=south] (FigA) at (0,0) {\includegraphics[height=3cm,trim=6cm 17.5cm 5cm 2.5cm,clip]{figures/fig_invivo/rat18/radial_symmetry_depth_stretch.png}};
        \spy [closeup,magnification=3] on ($(FigA)+(-0.465,+0.075)$) 
        in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.115,+0.020)$) 
        in node[largewindow,anchor=east]       at ($(FigA.west)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.435,-0.075)$) 
        in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
        \end{tikzpicture}
    }
    \subcaption{Radial Symmetry~\cite{heiles2022pala} from B-mode frames\label{fig:rat18:subfig1}}
    \end{minipage}
    \begin{minipage}[b]{\linewidth}
    \resizebox{\textwidth}{!}{
        \begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
        \node[anchor=south] (FigA) at (0,0) {\includegraphics[height=3cm,trim=6cm 17.5cm 5cm 2.5cm,clip]{figures/fig_invivo/rat18/mspcn_12x.png}};
        \spy [closeup,magnification=3] on ($(FigA)+(-0.465,+0.075)$) 
        in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.115,+0.020)$) 
        in node[largewindow,anchor=east]       at ($(FigA.west)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.435,-0.075)$) 
        in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
        \end{tikzpicture}
    }
    \subcaption{mSPCN~\cite{liu2020deep} with NMS from B-mode frames\label{fig:rat18:subfig2}}
    \end{minipage}
%\end{figure*}
%\begin{figure*}%[H]
    \centering
    \begin{minipage}[b]{\linewidth}
    \resizebox{\textwidth}{!}{
        \begin{tikzpicture}[x=6cm, y=6cm, spy using outlines={every spy on node/.append style={smallwindow}}]
        %
        \node[anchor=south] (FigA) at (1.0,0) {\includegraphics[height=3cm,trim=6cm 17.5cm 5cm 2.5cm,clip]{figures/fig_invivo/rat18/sgspcn_12x_143.png}};
        \spy [closeup,magnification=3] on ($(FigA)+(-0.465,+0.075)$) 
        in node[largewindow,anchor=north east] at ($(FigA.north west) - (0,0.02)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.115,+0.02)$) 
        in node[largewindow,anchor=east]       at ($(FigA.west)$);
        \spy [closeup,magnification=2] on ($(FigA)+(-0.435,-0.075)$) 
        in node[largewindow,anchor=south east] at ($(FigA.south west) + (0,0.02)$);
        \end{tikzpicture}
    }
    \subcaption{Our SG-SPCN with NMS from RF frames\label{fig:rat18:subfig3}}
    \end{minipage}
    %\begin{minipage}[b]{.6\textwidth}
    %    \subcaption{Cross-sectional %plot\label{fig:subfig5}}
    %\end{minipage}
    %\hfill
    %\begin{minipage}[b]{.3\textwidth}
    %    \resizebox{\textwidth}{!}{
    %    \includegraphics
    %    [height=3mm,trim=6mm 14.5mm 5mm %1.5mm,clip]
    %    {figures/fig_invivo/rat18/mean_frame.png}
    %    }
    %    \subcaption{Averaged B-mode frames\label{fig:subfig5}}
    %\end{minipage}
    %
    \caption{\textbf{In vivo results} showing the vascular structure of rat brains. The images show accumulated localizations with $R=8$ from 5 compounded waves in (\subref{fig:rat20:subfig1})~to~(\subref{fig:rat20:subfig2}) and $R=12$ from 3 compounded plane waves in (\subref{fig:rat18:subfig1})~to~(\subref{fig:rat18:subfig3}) each using 128 transducer channel data of $120\times800$ frames. Blue rectangles highlight magnified views for better comparison. %Examples using MB tracking can be found in the supplementary material. 
    The dataset is made available at \href{https://doi.org/10.5281/zenodo.7883227}{doi.org/10.5281/zenodo.7883227}.
    }
    \label{fig:rat18}
\end{figure*}


==> figures/fig_invivo_rat20.tex <==
\begin{figure}[!b]%[!h]
        \centering
        %\begin{minipage}[b]{\linewidth}
        %\resizebox{\textwidth}{!}{
	    %   \includegraphics[height=3mm,trim=4mm 17.5mm 5mm 2.5mm,clip]{figures/fig_invivo/rat20/mean_frame.png}
        %}
        %    \subcaption{Mean frame using B-mode frames as input data\label{fig:rat20:subfig0}}
        %\end{minipage}
        %\begin{minipage}[b]{\linewidth}
        %\resizebox{\textwidth}{!}{
	    %   \includegraphics[height=3cm,trim=5cm 17.5cm 17cm 1.5cm,clip]{figures/fig_invivo/rat20/radial_symmetry_8x.png}
        %}
        %    \subcaption{Radial Symmetry~\cite{heiles2022pala} using B-mode frames as input data\label{fig:rat20:subfig1}}
        %\end{minipage}
        \begin{minipage}[b]{\linewidth}
        \resizebox{\textwidth}{!}{
		  \includegraphics[height=3cm,trim=5cm 14.8cm 12cm 1.5cm,clip]{figures/fig_invivo/rat20/unet_8x_bmode_norm.png}
        }
            \subcaption{U-Net~\cite{van2020super} using B-mode frames as input\label{fig:rat20:subfig2}}
            \vfill
        \end{minipage}
        %\begin{minipage}[b]{\linewidth}
        %\resizebox{\textwidth}{!}{
		%  \includegraphics[height=3cm,trim=5cm 18.2cm 17cm 1.95cm,clip]{figures/fig_invivo/rat20/sgspcn_8x_bmode_norm.png}
        %}
        %    \subcaption{Our SG-SPCN~\cite{liu2020deep} using B-mode frames as input\label{fig:rat20:subfig3}}
        %\end{minipage}
        \begin{minipage}[b]{\linewidth}
        \resizebox{\textwidth}{!}{
	       \includegraphics[height=3cm,trim=5cm 14.8cm 12cm 1.5cm,clip]{figures/fig_invivo/rat20/sgspcn_8x.png}
        }
            \subcaption{Our SG-SPCN using RF-data frames as input\label{fig:rat20:subfig4}}
		\end{minipage}
        \caption{\textbf{In vivo rat-20 results} showing the vascular structure of a rat brain. The images are generated using accumulated localizations with upscale factor $R=8$. The data comprises 5 compounded waves using 128 transducer channel data from $120\times800$ frames without temporal tracking. %The dataset is made available at \href{https://doi.org/10.5281/zenodo.7883227}{doi.org/10.5281/zenodo.7883227}.
        }
        \label{fig:rat20:invivo}
\end{figure}


==> figures/fig_pala_sim.tex <==
% Simulation Results: Figure with cropped versions
\begin{figure*}[b]
  \centering
  \begin{minipage}[b]{0.120\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./figures/pala_sim_results/pala_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./figures/pala_sim_results/pala_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=1240 20 0 715, clip]{./figures/pala_sim_results/pala_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./figures/pala_sim_results/pala_ulm_img_15k_gam0.9_128chs.png}
    %\vspace{-.5cm}
    \subcaption{RS~\cite{heiles2022pala}\label{fig:method2}}
    %\vspace{+.1cm}
  \end{minipage}
  \hfill
    \begin{minipage}[b]{0.120\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./figures/pala_sim_results/gulm_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
        \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./figures/pala_sim_results/gulm_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
        \includegraphics[width=\textwidth,trim=1240 20 0 715, clip]{./figures/pala_sim_results/gulm_ulm_img_15k_gam0.9_128chs.png}\par\vspace{1mm}
        \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./figures/pala_sim_results/gulm_ulm_img_15k_gam0.9_128chs.png}
        %\vspace{-.5cm}
        \subcaption{GULM~\cite{gulm:2023}\label{fig:method3}}
        %\vspace{+.1cm}
    \end{minipage}
  \hfill
  \begin{minipage}[b]{0.120\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./figures/pala_sim_results/unet_8x_iq.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./figures/pala_sim_results/unet_8x_iq.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=1240 20 0 715, clip]{./figures/pala_sim_results/unet_8x_iq.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./figures/pala_sim_results/unet_8x_iq.png}
    \subcaption{U-Net~\cite{van2020super}\label{fig:method4}}
    %\vspace{+.1cm}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.120\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./figures/pala_sim_results/mspcn_8x_iq.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./figures/pala_sim_results/mspcn_8x_iq.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=1240 20 0 715, clip]{./figures/pala_sim_results/mspcn_8x_iq.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./figures/pala_sim_results/mspcn_8x_iq.png}
    \subcaption{mSPCN~\cite{liu2020deep}\label{fig:method5}}
    %\vspace{+.1cm}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.120\textwidth}
    \centering
    \includegraphics[width=\textwidth,trim=240 538 1030 238, clip]{./figures/pala_sim_results/sgspcn_8x_rf.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=310 45 980 750, clip]{./figures/pala_sim_results/sgspcn_8x_rf.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=1240 20 0 715, clip]{./figures/pala_sim_results/sgspcn_8x_rf.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth,trim=820 560 200 100, clip]{./figures/pala_sim_results/sgspcn_8x_rf.png}
    \subcaption{%\mbox{SG-SPCN}
    Ours\label{fig:method6}}
    %\vspace{+.1cm}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.120\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/gt_crop_1.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/gt_crop_2.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/gt_crop_3.png}\par\vspace{1mm}
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/gt_crop_4.png}
    \subcaption{GT\label{fig:method1}}
    %\vspace{+.1cm}
  \end{minipage}
  %\hfill
  \begin{minipage}[b]{0.233\textwidth}%.24\textwidth
    \raggedright
    {\scriptsize Counts [\#]}\hfill
    \vspace{-.8mm}
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/cross-section_1.pdf}\par\vspace{1mm}
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/cross-section_2.pdf}\par\vspace{1mm}
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/cross-section_3.pdf}\par\vspace{1mm}
    \includegraphics[width=\textwidth]{./figures/pala_sim_results/cross-section_4.pdf}
    \par\vspace{-2.5mm}
    \centering
    {\scriptsize Spatial dimension [px]}
    \par\vspace{-1mm}
    \subcaption{Cross-sectional views\label{fig:cross-section}}
    %\vspace{+.1cm}
  \end{minipage}
    \caption{\textbf{In silico ULM regions} from  Table~\ref{tab:benchmark} for localization assessment. The methods in (\subref{fig:method2})-(\subref{fig:method3}) are deterministic approaches whereas (\subref{fig:method4})-(\subref{fig:method6}) are based on deep learning networks with scale $R=8$. While ULM methods generally employ B-mode images, the results in (\subref{fig:method3}) and (\subref{fig:method6}) are generated from RF data in absence of computational beamforming. Our proposed SG-SPCN network renderings are found in (\subref{fig:method6}). Cross-sections are highlighted as white bars in (\subref{fig:method1}) and provided in (\subref{fig:cross-section}).} %(full frames in Suppl. Material)
    \label{fig:render_ulm_crop}
\end{figure*}


==> figures/fig_rf_localization/fig_rf_localization.tex <==
\begin{figure}
    \begin{minipage}{\linewidth}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=.9\linewidth]{figures/fig_rf_localization/2nd_attempt/result_lores_insilico_10+2.eps}
        \label{fig:sub:rf_insilico}
        \subcaption{\textit{In silico} test frame}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=.9\linewidth]{figures/fig_rf_localization/2nd_attempt/result_hires_insilico_10+2.eps}
        \label{fig:sub:rf_insilico_magnify}
        \subcaption{\textit{In silico} magnified region}
    \end{minipage}
    \vspace{.1cm}
    \end{minipage}
    \begin{minipage}{\linewidth}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=.9\linewidth]{figures/fig_rf_localization/1st_attempt/result_lores_invivo_8.eps}
        \label{fig:sub:rf_invivo}
        \subcaption{\textit{In vivo} frame}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=.9\linewidth]{figures/fig_rf_localization/1st_attempt/result_hires_invivo_8.eps}
        \label{fig:sub:rf_invivo_magnify}
        \subcaption{\textit{In vivo} magnified region}
    \end{minipage}
    \end{minipage}
    \caption{\textbf{RF frame localizations} from \mbox{SG-SPCN} predictions highlighted as red pixels in IQ signals from synthetic test and real data. Blue rectangles indicate the magnified region. These results demonstrate our network's capability to transfer knowledge about wavefronts learned from a synthetic training dataset to unseen \textit{in vivo} frames.}
    \label{fig:mb_localization}
\end{figure}

==> image_benchmark.tex <==
1. insilico frames
a) U-Net
b) Radial Symmetry 
c) MEMG-based PaCE
d) NGCC-based PaCE
e) Temporal filtered NGCC-based?

2. invivo frames
a) single wave emission (before temporal and after?)
b) three angles accumulation


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}


==> notes.tex <==
todo:
- BVM results?

done:
- arch figure: salmon to light pink

==> tables/tab_benchmark_sigvar.tex <==
\begin{tabularx}{\textwidth}{ 
         >{\raggedright\arraybackslash}p{9.5em} %| 
         >{\raggedright\arraybackslash}p{4em} %|
         >{\raggedleft\arraybackslash}p{2.75em} %|
         >{\raggedleft\arraybackslash}p{8em} %| 
         >{\raggedleft\arraybackslash}p{6em} %| 
         >{\raggedleft\arraybackslash}p{6em} %| 
         >{\raggedleft\arraybackslash}p{6em} %| 
         >{\raggedleft\arraybackslash}p{10em} %| 
         }
\toprule
Method & Input & Waves & {RMSE [$\lambda/10$]}~$\downarrow$ & {Jaccard~[\%]}~$\uparrow$ & {SSIM~[\%]}~$\uparrow$ & Weights [\#]~$\downarrow$ & Frame Time [ms]~$\downarrow$ \\
\midrule
Lanczos~\cite{heiles2022pala} & B-mode & 3 & $1.524\pm0.175$ & $38.688$ & $75.870$ & $0$ & $\text{T}_{\text{DAS}}$ + $0.382$ $\times$ 1$\mathrm{e}$3 \\
2-D Gauss Fit~\cite{song:2018} & B-mode & 3 & $1.240 \pm 0.162$ & $51.342$ & $73.930$ & $0$ & $\text{T}_{\text{DAS}}$ + $3.782$ $\times$ 1$\mathrm{e}$3 \\
RS~\cite{heiles2022pala} & B-mode & 3 & $1.179 \pm 0.172$ & $50.330$ & $72.170$ & $0$ & $\text{T}_{\text{DAS}}$ + $0.099$ $\times$ 1$\mathrm{e}$3 \\ %0.0992
%Spline~\cite{song:2018} & B-mode & $1.504\pm0.174$ & $39.370$ & $75.720$ & $0$ & $\text{T}_{\text{DAS}}$ + $0.277$ $\times$ 1$\mathrm{e}$3 \\
G-ULM~\cite{gulm:2023} & RF-data & 1 & $0.967\pm0.109$ & $78.618$ & $92.020$ & $0$ & $3.747$ $\times$ 1$\mathrm{e}$3 \\
\midrule
%
U-Net~\cite{van2020super} + NMS & B-mode & 3 & $0.565 \pm 0.078$ & $92.336$ & $93.345$ & $12982849$ & $\text{T}_{\text{DAS}}$ + $\text{T}_{R}$ + $80.384$ \\
%
%
{mSPCN~\cite{liu2020deep}} + NMS & B-mode & 3 & $0.696 \pm 0.097$ & $85.413$ & $93.653$ & $453568$ & $\text{T}_{\text{DAS}}$ + $3.269$ \\
{mSPCN~\cite{liu2020deep}} + NMS & RF-data & 3 & $1.093 \pm 0.197$ & $60.728$ & $92.191$ & $453568$ & $14.422$ \\
{SG-SPCN [Ours]} & B-mode & 3 & $0.664 \pm 0.098$ & $88.320$ & $93.080$ & $658496$ & $\text{T}_{\text{DAS}}$ + $3.116$ \\
{SG-SPCN [Ours]} & RF-data & 1 & $0.581 \pm 0.100$ & $88.915$ & $93.539$ & $658496$ & $6.520$ \\
{SG-SPCN [Ours]} & RF-data & 3 & $0.423 \pm 0.094$ & $90.012$ & $94.323$ & $658496$ & $16.989$ \\
%\midrule
%U-Net~\cite{van2020super} + NMS + RS & B-mode & 3 & $0.404 \pm 0.083$ & $92.479$ & $93.679$ & $12982849$ & $\text{T}_{\text{DAS}}$ + $\text{T}_{R}$ + $84.452$ \\
{SG-SPCN [Ours] + RS} & RF-data & 3 & $0.335 \pm 0.098$ & $90.036$ & $94.339$ & $658496$ & $32.070$ \\
%
%
\bottomrule
\end{tabularx}
